Negotiating Team Formation Using Deep Reinforcement Learning

When autonomous agents interact in the same environment, they must often cooperate to achieve their goals. One way for agents to cooperate effectively is to form a team, make a binding agreement on a joint plan, and execute it. However, when agents are self-interested, the gains from team formation must be allocated appropriately to incentivize agreement. Various approaches for multi-agent negotiation have been proposed, but typically only work for particular negotiation protocols. More general methods usually require human input or domain-specific data, and so do not scale. To address this, we propose a framework for training agents to negotiate and form teams using deep reinforcement learning. Importantly, our method makes no assumptions about the specific negotiation protocol, and is instead completely experience driven. We evaluate our approach on both non-spatial and spatially extended team-formation negotiation environments, demonstrating that our agents beat hand-crafted bots and reach negotiation outcomes consistent with fair solutions predicted by cooperative game theory. Additionally, we investigate how the physical location of agents influences negotiation outcomes.

==> LetterRevisionMinor.tex <==
Dear Editor, 

We are pleased to submit a minor revision of our paper "Negotiating Team Formation Using Deep Reinforcement Learning". 

The reviewers have asked for minor amendments, which we have now addressed. 


The key changes we have made are as follows: 
1) We have added a more thorough discussion of the existing literature connecting cooperative and competitive game theory.  In particular, we have added a subsection on related work regarding connections between the Shapley values and competitive and Nash equilibria in various games. We've cited all the papers suggested by the reviewers and several additional ones on this topic (see page 3, under the heading "The relation between the Shapley value and Nash equilibria"). 
2) We have added notes regarding the minor comments by the reviewers (e.g. adding to figure captions which of the environments they refer to, adding a note on the impact of the length of the episode)
3) We have corrected all the typos / grammar errors pointed out by the reviewers. 


Please find a detailed list of responses to the reviews below. 

We thank you again for your consideration!

Best regards, 
Yoram Bachrach (on behalf of the authors). 


Detailed changes (original comments included):



> Reviewer #1: The authors have provided convincing answers to the concerns risen in the first revision and introduced according modifications in the manuscripts to clarify these points for the readership. I have no further concerns and recommend to accept the manuscript for publication.

>> Thank you!



> Reviewer #2: This version of the manuscript is much improved from the last version. In the last version I had one main complaint that the paper was ignoring the connection between Nash equilibrium in the competitive game and Shapley value in the cooperative game. The authors have introduced a new section describing how to calculate a Nash equilibrium through backward induction in the competitive game and then compare this solution to the Shapley value in the cooperative game, showing that there is high correlation between the two. I think this section adds a lot to the paper, providing a link between RL, Nash equilibrium, and Shapley value. However, I would like to see more discussion on the historical work that has been done already on the connection between Shapley value and competitive equilibrium. For example the following papers seem highly relevant but are not cited: 
Shapley, L. S. (1964). Values of large games VII: a general exchange economy with money. Research Memorandum 4248-PR. RAND Corporation, Santa Monica, CA.
Aumann, R. J. (1975). Values of markets with a continuum of traders. Econometrica 43, 611-646
Aumann, R. J. and L. S. Shapley (1974). Values of Non-Atomic Games. Princeton: Princeton University Press.

>> Done. We have added a subsection in page 3 with a more thorough discussion of the existing literature connecting cooperative and competitive game theory.  We now cite all of the papers you suggested, as well as additional work tying Shapley values and Walrasian equilibria or tying the Shapley value to other bargaining solution concepts. 



> Additionally, this typo was not corrected from last time:
Pg 26: "negotiate how to split the spoils of their team achievement." instead of "negotiate how to the split the spoils of their team achievement."

>> Fixed



> Section 4.6 along with the other changes address most of my original concerns about the paper, but I would like to see a more thorough related works section that discusses the existing literature connecting cooperative and competitive game theory. 

>> Done (see previous comment, and page 3 in the paper)



> Reviewer #3: In this paper, the authors examine the behavior learned by reinforcement learning methods in multiagent weighted voting game environments and demonstrate a correlation between trained agent payoffs and Shapley values, a fairness/power solution concept from cooperative game theory. They determine that the specifics of negotiation protocol dynamics and/or RL learning dynamics can affect the degree to which agent payoffs correlate with Shapley values. They also confirm that a Nash equilibrium, at least for a very simple weighted voting environment, also has performance correlated (but not identical) with Shapley values. I believe that this paper takes an important initial step towards understanding a relatively under-explored problem at the intersection of RL and cooperative game theory. The paper is in general well-written and easy to follow.

I agreed with reviewer 2's comments questioning the link between Nash Equilibria and Shapley values. The addition of section 4.6, demonstrating that the two are at least correlated, is a solid and welcome addition to the paper, which in my mind, addresses these issues well enough. With the changes made thus far, I'd recommend this paper for acceptance.

>> Thank you. 



> I have minor notes as follows:
- Section 4.4 shows that agents placed further from patches are less able to leverage their higher weights to gain higher rewards due to increased difficulty in negotiations. Adding to this, it may be interesting to see how uniformly changing the difficulty of negotiation for all agents affects the correspondence between Shapley values and empirical reward shares. Negotiation difficulty could be uniformly increased by lowering the steps per episode in the Team Patches environment or lowering the probability of continuing, p, in the Propose-Accept environment. Perhaps agents with disproportionally high or low weights will diverge more from Shapley values when time is more limited for everyone to carry out negotiation.

Regardless, the experiment in section 4.4 shows that agent expected payoff is affected by negotiation protocol dynamics, and in section 4.6, the authors do note that the Nash equilibrium depends on the specific number of rounds in the modified Propose-Accept environment. The inclusion of such an additional experiment is not critical to my "accept" recommendation.

>> Added a short note (see page 20). Our results are fairly consistent when slightly perturbing the episode length. 



> - Page 17, Section 4.3.1, Figure 6 - which environment is this figure for (Propose-Accept or Team Patches)?

>> This is for propose-accept. We've added this to the caption.



> - Page 11, minor typos:
        Line 19: distribution to to a train set...
        Line 32: For instance, for certain distribution we are more likely...
        Line 37: reinforcement learning may no converge...

>> Fixed.


==> deleted.tex <==
\section{Abstract}
    1. Team formation is an important problem, but the existing methods to solve it require human data and thus will not scale. \\
    2. Thus we introduce a new method based on deep RL that does not require human data and so ought to scale. \\
  3. Our new method produces results that generally agree with those of game theory (Shapley value, etc). \\
    4. Now that we've established this new method, we apply it to even more complex situations where it would be intractable to produce a prediction from game theory (Markov games). We show that it still yields interesting results in this new setting. \\

AL: Can team formation be also an interesting thing to look at as more general mechanism for incentivizing co-operation among agents in MARL? If the only way for me to gain money is for someone to pick me, doesn't this act as a pressure for me to start playing with a a team spirit?? Can this be an explicit choice in every MARL environment? 


\section{Introduction}

that characterize a fair distribution of reward based on each agent's contribution
Maybe footnotes?
See \cite{brandenburger2007cooperative, chalkiadakis2011computational} for a review of relevant solution concepts.
Such indices reflect how negotiating agents are likely to share a joint budget or reward \citep{dubey1975uniqueness,gul1989bargaining}. Researchers noted that the true power of a participant may not be proportional to its weight \citep{banzhaf1964weighted,shapley1954method}.


Raise a question
Given such an interaction protocol, how should one construct a negotiating agent so as to maximize the reward obtained? Negotiators have to take into account that agents may have different skills, ability levels and preferences which are likely to be reflected in the agreed allocation of reward. 

However, many such approaches require human data and thus do not scale \citep{oliver1996machine,lin2010can}. Further, such bots are hand-crafted and tailored to a specific negotiation protocol, so modifying the protocol or switching to a different protocol require manually re-writing the bot \citep{rosenschein1994rules,jennings2001automated,an2010automated}. 

To address this, we propose a framework for training team formation negotiation agents capable of operating under many different negotiation protocols and with a number of other agents. Rather than relying on hand-crafted bots, built for a specific negotiation protocol, we propose training negotiation agents using multi-agent reinforcement learning (RL). By allowing multiple independent reinforcement learning agents to interact with one another using the target negotiation protocol, agents can learn to develop negotiation strategies based on the outcomes in the simulator. 
In contrast, we propose applying reinforcement learning (RL) to construct negotiation agents. 
Further, RL requires no human data and thus scales well. 
More importantly, when modifying or switching to a different negotiation protocol, the RL system can be trained based on episodes simulated on the new protocol to constuct agents for this new protocol, so the approach easily generalizes to new settings. 

\textcolor{red}{RE: Clean up these citations. At the moment they are meaningless. Also add additional citations for other points.}
YB - done
% ^^^ RE - Why is this now a footnote? ^^^

 Short summary of our solution to the flaws in the related work



Bullet points listing differences between the Markov game and characteristic function perspectives.
\begin{enumerate}
    \item Real world negotiation actions are temporally extended.
    
    \item Policies must implement strategic decisions.
    
    \item Strategic decisions are made only quasi-simultaneously since some information about what one player is starting to do can inform the others' decision and vice versa.
    
    \item  Decisions must be made despite only having partial information about the state of the world and the activities of the other players.
\end{enumerate}

Bullet points about learning to negotiate in the real world.
\begin{enumerate}
    \item Learning which high-level strategic decision to make often occurs simultaneously
with learning the low-level tactics relating to how to efficiently implement said decision.

    \item Implementing effective negotiation may or may not involve solving coordination subproblems, and the extent of coordination required may depend strongly on idiosyncratic features of the environment that are not easily captured in a characteristic function description.
    
    \item Some strategic situations may allow for multiple different implementations of negotiation policies that would be considered the same from the perspective of cooperative game theory. Moreover, these implementations may differ from one another in the extent to which they require coordination with one another.
    
    \item The complexity of learning how to implement effective negotiation policies may not all be the same as one another. For example, solely due to implementation complexity, it may be easier to implement a veto vote in a way that cannot be accounted for by adjusting the characteristic function description.
\end{enumerate}

Game theory is the branch of mathematics which analyzes interactions between self-interested agents, modelling strategic interactions between rational decision-makers \citep{osborne1994course}. {\em Cooperative} game theory focuses on interactions between agents who form teams and make enforceable agreements about the outcomes, such as agreements regarding sharing a joint reward \citep{brandenburger2007cooperative,chalkiadakis2011computational}. One model that has received significant attention is that of weighted voting games, where every agent has a weight, and an agent subset (called team or coalition) is successful if the sum of the weights of its participants exceeds a fixed threshold, typically half the total weight of all the agents \citep{banzhaf1964weighted,holler1982forming}. Weighted voting games offer a simple model of coalition formation in legislative bodies. For example, political parties who each have a certain number of parliament seats following an election, may need to form a coalition of multiple parties so as to achieve half of the total number of parliament seats in order to establish a ruling government \citep{leech2002designing,felsenthal1998measurement}. 

\subsection{Game Theory}


Researchers examining cooperative games have tried making predictions regarding the agreements negotiated by agents in such settings, proposing several {\em solution concepts}. Some such solutions, such as the core and nucleolus \citep{schmeidler1969nucleolus}, have focused on identifying stable agreements. Other solutions have tried to identify {\em fair} agreements between agents, reflecting the strength of the negotiation position of each agents, or measuring their relative ability to affect the outcome of the game. The most prominent of these is the Shapley value \citep{shapley1953value} which has been widely studied for weighted voting games \citep{shapley1954method, straffin1988shapley}. In particular, it has been used to estimate political power in legislative bodies \citep{shapley1954method,leech2002designing,felsenthal1998measurement}). 
%
Many methods based on game theoretic solutions have been proposed to predict agreements and outcomes in team formation negotiation settings \citep{hart1996bargaining,snyder2005legislative}, including some work that applies the Shapley value to predict outcome in such settings \citep{gul1989bargaining}, and work examining human negotiation data \citep{lin2010can,bachrach2011rip,mash2017form}
The Shapley value characterizes the fair contribution of agents in cooperative games such as weighted voting games. Given a weighted voting game $v = [(w_1, \ldots, w_n); t]$ it allocates 100\% of the reward among the agents, reflecting the fair amount each weight should get (i.e. proposes an allocation $\phi(v) = (\phi_1, \ldots, \phi_n)$ where $\sum_{i=1}^n \phi_i = 1$). 
Negotiation and team formation; 











\section{Introduction}
% Such domains require agents to negotiate with one another as to which course of action to take and how to share the derived rewards~\cite{zlotkin1994coalition,sandholm2000agents,jennings2001automated,faratin2002using,parsons2002game,nair2002team}. 
% RoboCUP rescue? 


% We refer to the task of forming an agent team and deciding how to distribute the gains from cooperation between the individual agents as the {\em team formation negotiation} process. 

%Many tasks require the cooperation between multiple agents, with many domains requiring whole teams of agents to coordination their actions in order to achieve a goal. 

% Researchers in the field of multi-agents systems have proposed many approaches for planning and coordinating the actions of agents, surveys of which can be found in various papers~\cite{kraus1997negotiation,stone2000multiagent,horling2004survey,ren2005survey,cao2013overview}.
% transferable utility




% TODO: YB - connect this to cooperative game theory, and coalition structure generation

% Example from politics here? Is there a more DeepMind multiagent domain we can describe here? 


% \paragraph{Example real world problem}

% We refer to the process of constructing the team of agent as the {\em team formation} process, and the process of deciding how to distribute the joint reward between the agents as the {\em reward allocation} process.



One example of such a domain that has been widely investigated is the formation of a coalition government following an election. Consider a set of political parties who each obtained a certain number of parliament seats in an election, and where a quota of the majority of the seats is required to form a ruling government. If no single party has won the majority of the votes on its own, multiple parties would have to join so as to form a ruling government. Parties in this setting would have to negotiate to form a ruling government.
This is rare in the UK, and has probably never happened in the USA, but is the typical situation in many other countries. 
% 
For intuition, consider a parliament of 100 seats, two big parties with  
49 seats each and a small party with 2 seats; a majority requires 50 seats (half of the total number of seats), so no party can form a government on its own. While each big party far more seats than the small party, any team of two or more parties has the required majority of seats. Under such a framing of the domain, any team of at least two out the three agents is sufficient for completing the task of forming a government, and due to this symmetry between agents one may claim they all have equal power. 

% RL is good and strong, so it makes sense to use it to construct good strong negotiating agents. 

% One potential caveat is that RL methods are designed for stationary enviroments, whereas each negotiator faces opponents who may adjust their behavior, making the environment non-stationary. 

\section{Banzhaf Index}
\textcolor{red}{Richard: Currently removed as we don't look into the Banzhaf index at all. My suggestion, remove entirely.}
The {\em Banzhaf index}~\cite{banzhaf1964weighted} measures the proportion of coalitions that an agent is critical in, out of all the coalitions containing that agent. It is given by the vector $\beta(v) = (\beta_1(v), \beta_2(v), \ldots, \beta_n(v))$ where:
 $\beta_i(v) = \frac{1}{2^{n-1}}  \sum_{C \subseteq A | i \in C} [v(C) - v(C \setminus \{a\})]$. 

\section{Propose-Accept Environment}
\textcolor{red}{Richard: Currently removed as it is way too long. May include the figure and some words in the experiments section, but at the moment it's a page dedicated to explaining a basic use case of the environment. This is important, just needs to be shorter.}
\label{l_sect_propose_accept_env}

We first investigate whether agents trained on the propose-accept environment tend to reach agreement, and the overall total utility agents achieve in each episode. For each of the $k$ boards, we construct $t=200$ sets of agents trained using independent RL. Each set consists of $n=5$ agents, each trained with the other agents in the team, for a total of $m=500,000$ episodes. Each training episode is executed using a different board sampled at random from the board distribution $D$. Thus, for each of the $k$ evaluation boards, we generate $t=200$ sets of co-trained co-trained negotiator agents. Each evaluation board is inspected by executing an evaluation step after every $5,000$ training episodes. During such an evaluation step, we let each of the $t=200$ agent sets generated for that evaluation board play $5,000$ episodes on that board (without executing any learning updates). This allows us to estimate the expected behavior of a set of independent RL agents, trained on random boards from a distribution $D$ when playing on the target evaluation board. 

The propose-accept game is highly stochastic, as the next proposer is chosen at random, and as the decision regarding the termination of an episode following a declined proposal is also random. Although there is high uncertainty regarding the outcome of any single game, our results are based on averaging the outcomes of $5,000$ games, allowing use to accurately estimate the expected outcomes. Clearly, the average amount an agent can win when playing the same board depends on its weight in that board. An agent who is assigned a high weight is in a better position than an agent who is assigned a low weight in the board. 

Figure~\ref{fig:single_board_eval} shows the amount won per episode for each weight in the the board $[(5, 6, 7, 5, 4); 15]$. As the figure indicates, higher weights achieve a higher reward (average over many episodes player on this board and across different sets of negotiator agents). This is not surprising, since a higher weight gives a player more negotiation power, as they have more potential teams they can form. Perhaps more interestingly, the figure also shows that agents reach in agreement in almost all rounds even early on in the training process. Further, most episodes end after very few proposal turns. 

\begin{figure}[htbp]                
\centering
\includegraphics[width=0.5\paperwidth]{images/prop-accept-single-board-eval.png}
\caption{Evaluation on a single board}
\label{fig:single_board_eval}
\end{figure}
% TODO:YB: Better make a boxpolot for each weight, at a specific timestep!

\section{Beating Baseline Bots}
\textcolor{red}{Richard: Removed as there isn't space. My suggestion is to reduce this a lot and include it in the appendix.}

The above results indicate that independent RL agents many to reach an agreement often. When agents fail to reach an agreement they obtain no reward, so agents who almost never reach an agreement would be bad negotiators. However, reaching agreement easily by itself does not make an agent a strong negotiator. For instance, an agent who accepts any offer is likely to reach agreement easily but perform poorly, as they would take even very low offers (even when they have a high relative weight and thus a strong negotiation position). The key advantage of using our approach is not needing to hand-craft bots for a specific negotiation protocol. We now investigate the performance of independent RL agents against heuristic hand-crafted bots designed for this negotiation protocol. 

There are two types of decisions agents in the propose-accept environment have to make: when they are the proposer, they need to decide which viable team to propose and how to allocate the total reward among the team members, and when they are a proposee, they have to decide whether to accept or decline the offer. 

Our simplest baseline is a {\em random bot}. As a proposer, it selects an allowed proposal uniformly at random from the set of all such proposals. As a proposee it accepts with probability $\frac{1}{2}$ and rejects with probability $\frac{1}{2}$. 

Another baseline is the {\em weight-proportional bot}. 
As a proposer, it chooses a viable team $C$ which contains itself from the set of all such teams. It then proposes an allocation of the reward that is proportional to each the team agents' weights. Formally, given a board $[(w_1, \ldots, w_n); q]$, we denote the total weight of a team $C$ by $w(C) = \sum_{i \in C} w_i$. For the team it chose, the bot uses the target allocation $p_i = \frac{w_i}{w(C)} \cdot r$ where $r$ is the fixed total reward. \footnote{Our framework's action space includes only integral reward allocations, so the bot proposes chooses the integral reward allocation that minimizes the $L_1$ distance to the target allocation.} 
As a proposee, the bot computes its share of the same target allocation $p_i = \frac{w_i}{w(C)} \cdot r$ in the proposed team $C$, and compares it with the amount $r_i$ offered to it in the proposal. We denote by $g_i = r_i - p_i$ the amount by which the offer $r_i$ exceeds $p_i$, the bot's expectations under the weight-proportional allocation. A high positive amount $g_i$ indicates that the bot is offered much more than it believes it deserves according to the weight-proportional allocation, while a negative amount indicates it is offered less than it thinks it deserves (when offered exactly the weight-proportional share we have $g_i = 0$). The probability of the bot accepting the offer is $\sigma(c \cdot g_i)$ where $\sigma$ denotes the logistic function $\sigma(x)=\frac{1}{1+e^{-x}}$, and where $c=5$ is a constant correcting the fact that $g_i$ only ranges between $-1$ and $+1$ rather than between $- \infty$ and $+ \infty$. Thus the bot accepts a ``fair'' offer (according to the weight-proportional target) with probability of $\frac{1}{2}$, and the probability convexly increases as $g_i$ increases (and decreases as $g_i$ decreases). 
% TODO: YB: rewrite a bit more formally... 

Similarly to the procedure in Section~\ref{l_sect_propose_accept_env}, for each evaluation board we construct many agent teams. For our comparison between the hand-crafted bot and RL agents, for each evaluation board, we create $t=200$ {\em pairs} of agent team, where in each pair we have one group of $n=5$ independent RL agents (called the {\em all-RL group}, and one set consisting of 1 bot and 4 independent RL agents (called the {\em single-bot group}. Similarly to the previous experiment each group is co-trained for $m=500,000$ episodes (each episode using a different board sampled at random from the board distribution $D$); again, similarly to before, during an evaluation step, we let each agent group play $5,000$ games episodes on the evaluation board. We repeat the same analysis, each time allowing the bot to play a different weight in the board (i.e. letting the bot be the agent in the first position, in the second position and so on).

We focus on the performance of the RL agent from the all-RL group and the bot from the single-bot group, when playing the same weight on the same evaluation board. We average the fraction of the total fixed reward achieved by the RL-agent and bot over the $t=200$ group pairs and over the $5000$ episodes played with each evaluation board, and examine the difference $d$ between the amount won by the RL-agent and the amount won by the bot. A positive value for $d$ indicates the RL-agent has a better performance than the bot, and a negative number shows a higher performance for the bot. Figure~\ref{fig:weight-bot-run} shows the difference $d$ on runs for the board $[(5, 6, 7, 5, 4); 15]$ (same as the previous experiment). 

\begin{figure}[htbp]                
\centering
\includegraphics[width=0.5\paperwidth]{images/weight-bot-run-.png}
\caption{Performance of independent RL-agents versus the weight-proportional hand-crafted bot}
\label{fig:weight-bot-run}
\end{figure}

The figure shows that even when training only for a short amount of time, the RL-agent has either the same or superior performance as the bot. On average (across boards and episodes played on each evaluation board), the RL-agent outperforms the bot, achieving 2.5\% more of the total reward. We performed a Mann-Whitney-Wilcoxon test to check \footnote{This is a non-parametric test similar to Student's T-test, but resistant to deviations from a Guassian distribution.}, which shows the difference is significant at the $p<0.001$ level. 

Our results indicate that independent-RL trained agents can beat various heuristic hand-crafted bots, without requiring designing a bot specific to a given negotiation protocol. The propose-accept protocol is a very simple team formation negotiation environment, with extremely simple negotiation rules, making it relatively easy to construct hand-crafted bots for the domain. While our experiments certainly do not rule out the existence of other bots who may outperform independent RL-agents, we feel that the above results (with reasonable heuristic bots) indicate that our technique offers a way of automatically constructing at least reasonable negotioators, without requiring fitting a bot to a given negotiation protocol. 

\section{Converge to the Shapley Value}
As the Shapley value was proposed as a ``fair'' solution, one might view this as studying whether independent-RL agents are likely to converge to fairly share the joint gains from cooperation.

Our environment is highly stochastic, so two episodes on the same board may result in very different outcomes. For instance, in two episodes on the same board, the chosen team in one episode might be completely different than the one chosen in the other episode.
yielding very different reward allocations.
Although we have a high uncertainty about the outcome of any {\em single} episode in our environment, once a team of RL-agents has been trained, we can examine the average rewards they obtain over {\em many} episodes on the same board. We can thus check whether the Shapley value is a good predictor of the average amount our agents would win on a board. In other words, one might ask whether RL agents typically converage to a fair allocation of the rewards (as interperted by the Shapley value from cooperative game theory). 

% Game theory offers various solution concepts that allow making predictions as to the outcome of negotiation and bargaining situations involving multiple self-interested agents. Our setting is one where agents have to form teams to achieve their goal and obtain a reward, and the key questions are which team would form and how would the agents agree to share the total reward between them. 

\section{Other}
Random sections cut from the text.
% \begin{figure}[htbp]
% \centering
% \begin{subfigure}{.32\textwidth}
%   \includegraphics[width=.95\linewidth]{images/.png}
%   \caption{Base Environment}
%   \label{fig:env_propose_accept_1}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \includegraphics[width=.95\linewidth]{images/.png}
%   \caption{Example 1}
%   \label{fig:env_propose_accept_2}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%   \includegraphics[width=.95\linewidth]{images/.png}
%   \caption{Example 2}
%   \label{fig:env_propose_accept_3}
% \end{subfigure}
% \caption{Propose-Accept environment.}
% \label{fig:env_propose_accept}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}{.48\textwidth}
%   \includegraphics[width=.45\linewidth]{images/shapley-points.png}
%   \includegraphics[width=.45\linewidth]{images/shapley-contour.png}  
%   \caption{Propose Accept}
%   \label{fig:propose_accept_shapley}
% \end{subfigure}
% \begin{subfigure}{.48\textwidth}
%   \includegraphics[width=.45\linewidth]{images/shapley-points.png}  \includegraphics[width=.45\linewidth]{images/shapley-contour.png}
%   \caption{Team Patches}
%   \label{fig:team_patches_shapley}
% \end{subfigure}
% \caption{Shapley points and contours.}
% \label{fig:shapley_points}
% \end{figure}



% \begin{figure}[h]
% \centering
% \begin{subfigure}{.48\textwidth}
%   \includegraphics[width=.45\linewidth]{images/shapley-points.png}  \includegraphics[width=.45\linewidth]{images/shapley-contour.png}
%   \caption{Shapley points and contour.}
%   \label{fig:team_patches_shapley}
% \end{subfigure}
% \begin{subfigure}{.48\textwidth}
%   \includegraphics[width=.95\linewidth]{images/prop-accept-single-board-eval.png}  
%   \caption{Effects of Spatial}
%   \label{fig:spatial_eval}
% \end{subfigure}
% \caption{Team Patches}
% \label{fig:team_patches_results}
% \end{figure}


% $v = [(5, 6, 7, 5, 4); 15]$. The Shapley values for the game $v$ are given by 
%$\phi_v = (\frac{1}{6}, \frac{1}{4}, \frac{1}{4}, \frac{1}{6}, \frac{1}{6})$. We note that although players 1, 2 and 5,



\subsection{Experiment 1: Bot Results}  % Rename. 
To begin, we evaluate our agents in Propose-Accept against a hand-crafted bot, demonstrating that it is good.  \textcolor{red}{Yoram: Fill all of this in.}

% \begin{wrapfigure}[8]{r}{15em}
%     \centering
%     \includegraphics[width=8em]{images/weight-bot-run-.png} 
%     \caption{(Placeholder) Bot results. \woj{Much bigger font, bigger picture, maybe white background (seaborn 'ticks' style looks nice)}}
%     \label{fig:bots}
% \end{wrapfigure}

The figure shows that even when training only for a short amount of time, the RL-agent has either the same or superior performance as the bot. On average (across boards and episodes played on each evaluation board), the RL-agent outperforms the bot, achieving 2.5\% more of the total reward. We performed a Mann-Whitney-Wilcoxon test to check \footnote{This is a non-parametric test similar to Student's T-test, but resistant to deviations from a Gaussian distribution.}, which shows the difference is significant at the $p<0.001$ level. 

Our results indicate that RL trained agents can beat various heuristic hand-crafted bots, without requiring designing a bot specific to a given negotiation protocol. The propose-accept protocol is a very simple team formation negotiation environment, with extremely simple negotiation rules, making it relatively easy to construct hand-crafted bots for the domain. While our experiments certainly do not rule out the existence of other bots who may outperform independent RL-agents, we feel that the above results (with reasonable heuristic bots) indicate that our technique offers a way of automatically constructing at least reasonable negotiators, without requiring fitting a bot to a given negotiation protocol.



\subsection{Experiment 2: Convergence to the Shapley value} % Rename to: Comparison to Game Theoretic Solutions? Consistency with Game Theory?
In this experiment, we investigate whether our agents trained to negotiate behave in a way that is consistent with solution concepts from cooperative game theory, focusing on the Shapley value. As the Shapley value was proposed as a ``fair'' solution, one can view this as studying whether independent-RL agents are likely to converge to fairly sharing the joint gains from cooperation.

To do this, we... .

We denote the the amounts won by weight $i$ on board $j$ in the evaluation as $s^j_i$ (these are the values averaged over the different agent groups and episodes played on board $v^j$), and refer to these as {\em empirical agent rewards}. Given the game $v^j$ we can also compute the Shapley values for the game $v^j$, denoted as $\phi(v^j) = (\phi^j_1, \ldots, \phi^j_n)$. We view $\phi^j_i$ as the game theoretic prediction of the fair share the agent with weight $w^j_i$ should get in a negotiation in the game $v^j$. As we have $n=5$ weights in our boards (and thus have 5 agents participating in every game), for each board $v^j$ we have $n=5$ Shapley values $\phi^j_1, \ldots, \phi^j_5$, and $n=5$ empirical agent rewards $s^j_1, \ldots, s^j_5$. We attempt to determine how well the values  $s^j_i$, reflecting how much the agent co-trained in a group of independent RL-agents has actually won, match the values $\phi^j_i$,  reflecting the game theoretic predictors of the fair amount an agent playing the weight should win.


We can apply this analysis to each of the $k$ boards, and obtain $k \cdot n$ pairs $\{ (\phi^j_i, s^j_i) \}_{i \in [n], j \in [j]}$ of a Shapley value fair share prediction and the empirical agent reward.


Figure~\ref{fig:shapley} shows the winnings by agents playing each weight on a specific evaluation board $v^j = [(w^j_1, w^j_2, \ldots, w^j_n); q]$, averaged across many episodes played on that board and over many groups of co-trained independent-RL agents. We use these values to estimate the expected reward a negotiation agent playing each weight would achieve when training agents using independent-RL. 


Figure~\ref{fig:shapley_points} shows a scatter plot of these pairs, where the x-axis is the Shapley value based fair share prediction, and the y-axis is the empirical reward of the RL co-trained agents.

% \footnote{Note that as there are $n=5$ agents, there are at most $5! = 32$ possible Shapley values, and as some Shapley values are much more common than others (due to our distribution of generated boards), points only occur in few locations on the x-axis.}
The figure indicates a strong correlation between the Shapley values of weights and the empirical gains of independent RL trained negotiator agents. 

\begin{figure}[htbp]
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[height=9em]{images/shapley-points.png}
  \includegraphics[height=9em]{images/shapley-contour.png}  
  \caption{Propose-Accept. \textcolor{red}{(@\textbf{Yoram}: wrong exp id?)} }
  \label{fig:propose_accept_shapley}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[height=9em]{images/spatial_shapley.png}  
  \includegraphics[height=9em]{images/spatial_contour.png}
  \caption{Team Patches. \textcolor{red}{(Need to re-run.)}}
  \label{fig:team_patches_shapley}
\end{subfigure}
\caption{Share of reward received by agents in both environments. Shapley points (left) and contours (right). Black line is W. Red line is X. Blue dots are Y, contours and Z. \textcolor{red}{Explanation}}
\label{fig:shapley}
\end{figure}




\textcolor{red}{Richard: Rewrite this.}
Figure~\ref{fig:propose_accept_shapley} depicts density-estimation contours. It shows that the majority of the mass occurs in close proximity to the $y=x$, indicating a good fit between the game theoretic prediction and the point to which our RL agents converge to. For our choice of a board distribution, most players have relatively equal Shapley values, with most of Shapley values falling close to $\frac{1}{n}$ (the Shapley value of players who have completely equal power). As the figure shows, for these cases our RL agents behave in a way that very closely matches the game theoretic fair prediction. For the rarer boards where there are players with significantly more power or significantly less power than others (i.e. boards where there is a high inequality in Shapley values), the RL-agents exibit a stronger deviation from the game theoretic ``fair'' reward. While for these cases the high-Shapley weights do empirically get a higher share of the rewards than low-Shapley weights, the gap in empirical reward is lower than the one predicted by game theory. In other words, ``strong'' players (according to the game theoretic prediction) do get a higher share than weak players, but not to the extent predicted; for these rare boards, the empirical allocation of reward achieved by the RL-agents is more equal than predicted by the Shapley value. 
% YB: TODO: Is there a better way to phrase this?

% \paragraph{Team Patches}
\textcolor{red}{RE: Team Patches}

To conclude, our analysis indicates that independent RL negotiation agents empirically achieve rewards that are consistent with the outcomes predicted by the Shapley value from cooperative game theory. Notably, this consistency extends to our proposed spatial negotiation environment even with its different negotiation protocol and spatial interactions. In Section~\ref{l_sect_shapley_distil} we investigate potential reasons for the variations which exist where some of the players are relatively weak and others are particularly strong. 

For the non-spatial environment, one may use tabular approaches when training on a single weight configuration (board); when agents need to generalize to previous unobserved boards requires using a function approximator for the value function, and we apply SARSA~\citep{SuttonBarto18} with a deep neural network as a function approximator (we use a deep neural network, an MLP with 3 hidden layers and a hidden layer size of 64). For the spatial environment, we use asynchronous advantage actor-critic (A3C) agents~\citep{mnih2016asynchronous}, where the spatial observations are first processed using a convolutional neural network followed by a deep neural network.


{\color{red}
Non-Spatial: SARSA with DNN for a Q function-approximator; 
Spatial: A3C.

Appendix:\\
Configuration of the DNN (number of layers, hidden, Adam optimizer; initialization?)\\
Configuration of the A3C - appendix.
}

\section{Converge to the Shapley Value}
As the Shapley value was proposed as a ``fair'' solution, one might view this as studying whether independent-RL agents are likely to converge to fairly share the joint gains from cooperation.

Our environment is highly stochastic, so two episodes on the same board may result in very different outcomes. For instance, in two episodes on the same board, the chosen team in one episode might be completely different than the one chosen in the other episode.
yielding very different reward allocations.
Although we have a high uncertainty about the outcome of any {\em single} episode in our environment, once a team of RL-agents has been trained, we can examine the average rewards they obtain over {\em many} episodes on the same board. We can thus check whether the Shapley value is a good predictor of the average amount our agents would win on a board. In other words, one might ask whether RL agents typically converage to a fair allocation of the rewards (as interperted by the Shapley value from cooperative game theory). 

(i.e. for a proposal $(r_1, \ldots, r_n)$, the agent $i$ obtains reward $r_i$, so all agents who are not members of the proposed team get a reward of zero)

Every agent apart 

At a distance of 2, the moved agent is the furthest agent from the patches, and as we continue to move it further back its share of the total reward continues to drop.

